Search for the pentaquark resonance signature in lattice QCD

Claims concerning the possible discovery of the \Theta^+ pentaquark, with minimal quark content uudd\bar{s}, have motivated our comprehensive study into possible pentaquark states using lattice QCD. We review various pentaquark interpolating fields in the literature and create a new candidate ideal for lattice QCD simulations. Using these interpolating fields we attempt to isolate a signal for a five-quark resonance. Calculations are performed using improved actions on a large 20^3 x 40 lattice in the quenched approximation. The standard lattice resonance signal of increasing attraction between baryon constituents for increasing quark mass is not observed for spin-1/2 pentaquark states. We conclude that evidence supporting the existence of a spin-1/2 pentaquark resonance does not exist in quenched QCD.

==> LATTECH/litrev_tab.tex <==

\newpage


\begin{sidewaystable}[h]     
\label{litrev:tab}     
\caption{ A summary of the current pentaquark studies in lattice QCD. This table summarizes the fields used, a brief description of the analysis techniques
          and the suggested quantum numbers of the $\theta^{+}$ if evidence was found. }
\begin{ruledtabular} 
\begin{tabular}{l|l|l|l}
Group & Int. Fields & Analysis Methods & Observations \cr
\hline
{\small B. Lasscock {\it et al.} } & $\chi_{NK},\chi_{\widetilde{NK}},\chi_{SS},\chi_{\widetilde{SS}}$ &
{\small  $2 \times 2$ Corr. Matrix                      }    &{\small no bound states found } \cr
     &    & {\small   Mass Splittings Analysis with     }    &{\small $0,1(\frac{1}{2}^{\pm})$ degenerate w/ $NK^{*},N(1535)K,N(1535)K^{*}$ } \cr
     &    & {\small   $NK,NK^{*},N(1535)K,N(1535)K^{*}$ }    &{\small $0,1(\frac{1}{2}^{\pm})$ NK scattering state} \cr
\hline
%
{\small F. Csikor {\it et al.} \cite{cis} } & $\chi_{NK},\chi_{\widetilde{NK}}$  &{\small $2 \times 2$ Corr. Matrix } &
{\small $0(\frac{1}{2}^{-})$ NK degenerate state } \cr
     &    &  Mass Ratio with NK  & $0(\frac{1}{2}^{-})$ Excited state, $0(\frac{1}{2}^{+})$ too massive \cr
\hline
%
{\small S. Sasaki \cite{sas} } & $\chi_{\widetilde{PS}}$  & {\small Standard Analysis } &{\small $0(\frac{1}{2}^{-})$ above s-wave NK }\cr 
     &    &   &  {\small  $0(\frac{1}{2}^{+})$ above p-wave NK }\cr
\hline
%
{\small N. Mathur {\it et al.} \cite{kent} }& $\chi_{NK},\chi_{\widetilde{NK}}$  & {\small Vol. Dep, Bayesian Analysis } &
{\small $0,1(\frac{1}{2}^{-})$ NK scattering state   } \cr
     &    &   & 
{\small $0,1(\frac{1}{2}^{+})$ p-wave NK degenerate    } \cr 
\hline
%
{\small N. Ishii  {\it et al.} \cite{ishi}} & $\chi_{\widetilde{PS}}$ & Hybrid BC & {\small $0(\frac{1}{2}^{-})$ NK scattering state  } \cr
     &    &   &  $0(\frac{1}{2}^{+})$ too massive  \cr
\hline
%
{\small T. T. Takahashi {\it et al.} \cite{tak} } & $\chi_{NK},\chi_{\widetilde{NK}}$ & $2 \times 2$ Corr. Matrix, Vol. Dep &
{\small $0(\frac{1}{2}^{-})$ NK scattering state }\cr
     &    &   &
{\small $0(\frac{1}{2}^{-})$ Excited not the NK scattering state }\cr
     &    &   &
{\small $0(\frac{1}{2}^{+})$ $N(1535)K$ Scattering State}\cr
\hline
%
{\small T. W. Chiu  {\it et al.} \cite{CHIU} }& $\chi_{NK},\chi_{\widetilde{NK}}
\footnote{The NK-style fields used by T. W. Chiu  {\it et al.} differs by a $\gamma_{5}$ in the nucleon part of the operator to the other groups listed.
The only effect of this is to reverse the intrinsic parity of the operator.}
,\chi_{\widetilde{PS}}$, & $3 \times 3$ Corr. Matrix &  {\small $0(\frac{1}{2}^{-})$ NK scattering state }\cr
     &    &   & {\small Ground state $0(\frac{1}{2}^{-})$ less massive than $0(\frac{1}{2}^{+})$} \cr
%
\end{tabular}
\end{ruledtabular}
\end{sidewaystable}
\newpage

==> TF_I0.neg/MassS/tab.tex <==
\begin{table}[h]
\caption{\label{tab:difI0.neg}
	Mass differences between the $I(J^P)=0(\frac{1}{2}^-)$
	pentaquark (colour singlet $NK$ and pseudoscalar-scalar diquark)
	states and the S-wave $N+K$ two-particle state.}
\begin{ruledtabular} 
\begin{tabular}{c|ccc}
$\kappa$ & $m_{\pi}^{2}({\rm GeV}^{2})$ & $aM_{NK} - aM_{N+K}^{\rm S-wave}$ & $aM_{PS} - aM_{N+K}^{\rm S-wave}$ \cr \hline
1.2780 &  0.693      & 0.056(10)  & 0.019(25)  \cr
1.2830 &  0.594      & 0.052(11)  & 0.019(30)  \cr
1.2885 &  0.487      & 0.048(13)  & 0.027(36)  \cr
1.2940 &  0.380      & 0.043(17)  & 0.062(53)  \cr
1.2990 &  0.283      & 0.026(30)  & 0.160(118) \cr
1.3025 &  0.213      & --0.011(67) & 0.381(335) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I0.neg/tab.tex <==
\begin{table}[ht]
\caption{\label{tab:I0.neg}
	Masses of the $I(J^P)=0(\frac{1}{2}^-)$ colour singlet $NK$
	and pseudoscalar-scalar diquark-type pentaquark states for
	various values of $\kappa$, compared with the masses of the
	S-wave $N+K$, $N+K^*$ and $N'+K$ two-particle states.}
\begin{ruledtabular}
\begin{tabular}{c|ccccc}
$\kappa$ & $aM_{NK}$ & $aM_{PS}$
	 & $aM^{\rm S-wave}_{N+K}$ & $aM^{\rm S-wave}_{N+K^*}$
	 & $aM^{\rm S-wave}_{N'+K}$			\cr \hline
1.2780 & 1.612(17)  & 1.576(22)  & 1.556(9)  & 1.762(14) & 2.180(27)  \cr
1.2830 & 1.539(17) & 1.508(27)  & 1.487(10) & 1.704(16) & 2.136(32)  \cr
1.2885 & 1.449(20) & 1.434(35)  & 1.406(12) & 1.635(19) & 2.093(39)  \cr
1.2940 & 1.345(28) & 1.381(51)  & 1.317(17) & 1.561(26) & 2.061(55)  \cr
1.2990 & 1.236(50) & 1.383(108) & 1.219(30) & 1.485(40) & 2.056(87)  \cr
1.3025 & 1.145(67) & 1.524(318) & 1.140(46) & 1.421(68) & 2.093(144) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I0.neg/tab4.tex <==
\begin{table}[h]     
\caption{\label{tab:I0.neg}
	Masses of the $I(J^P)=0(\frac{1}{2}^-)$ colour singlet $NK$,
	colour fused $NK$
	and pseudoscalar-scalar diquark-type pentaquark states.
	Mass differences between the $I(J^P)=0(\frac{1}{2}^-)$
	pentaquark (colour singlet $NK$ and pseudoscalar-scalar diquark)
	states and the S-wave $N+K$ two-particle state.
	And the masses of the
	S-wave $N+K$, $N+K^*$ and $N'+K$ two-particle states.
	for various values of $\kappa$. }
\begin{ruledtabular} 
\begin{tabular}{c|cccccccc}
$\kappa$ & $aM_{NK}$ & $aM_{PS}$ & $aM_{\widetilde{NK}}$
         & $aM_{NK} - aM_{N+K}^{\rm S-wave}$ & $aM_{PS} - aM_{N+K}^{\rm S-wave}$
	 & $aM^{\rm S-wave}_{N+K}$ & $aM^{\rm S-wave}_{N+K^*}$
	 & $aM^{\rm S-wave}_{N'+K}$			\cr \hline
\hline
1.2780 & 1.61(2) & 1.61(2) & 1.58(2) & 0.06(1) & 0.02(3) & 1.55(1) & 1.76(1) & 2.18(3) \cr
1.2830 & 1.54(2) & 1.54(2) & 1.51(3) & 0.05(1) & 0.02(3) & 1.48(1) & 1.70(2) & 2.14(3) \cr
1.2885 & 1.45(2) & 1.45(2) & 1.43(4) & 0.05(1) & 0.03(4) & 1.40(1) & 1.64(2) & 2.09(4) \cr
1.2940 & 1.35(3) & 1.37(3) & 1.38(5) & 0.04(2) & 0.06(5) & 1.31(2) & 1.56(3) & 2.06(5) \cr
1.2990 & 1.24(5) & 1.26(4) & 1.38(11) & 0.03(3) & 0.16(12) & 1.22(3) & 1.49(4) & 2.06(9) \cr
1.3025 & 1.14(7) & 1.11(11) & 1.52(32) & -0.01(7) & 0.38(33) & 1.13(5) & 1.42(7) & 2.09(14) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I0.pos/MassS/tab.tex <==
\begin{table}[h]
\caption{\label{tab:difI0.pos}
	Mass differences between the $I(J^P)=0(\frac{1}{2}^+)$
	pentaquark ($NK$ and pseudoscalar-scalar diquark)
	states and the P-wave $N+K$ two-particle state.}
\begin{ruledtabular}
\begin{tabular}{c|cc}
$\kappa$ & $aM_{NK} - aM^{\rm P-wave}_{N+K}$
	 & $aM_{PS} - aM^{\rm P-wave}_{N+K}$	\cr\hline
1.2780 & 0.231(28)  & 0.169(33) \cr
1.2830 & 0.225(33)  & 0.175(37) \cr
1.2885 & 0.215(41)  & 0.184(44) \cr
1.2940 & 0.197(56)  & 0.193(55) \cr
1.2990 & 0.166(88)  & 0.192(80) \cr
1.3025 & 0.112(135) & 0.184(128) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I0.pos/tab.tex <==
\begin{table}[h]
\caption{\label{tab:I0.pos}
	Masses of the $I(J^P)=0(\frac{1}{2}^+)$ $NK$ and
	pseudoscalar-scalar diquark-type pentaquark states for various
	values of $\kappa$, compared with the masses of the P-wave $N+K$,
	S-wave $N^*+K$ and P-wave $N+K^*$ two-particle states.}
\begin{ruledtabular} 
\begin{tabular}{c|ccccc}
$\kappa$ & $aM_{NK}$ & $aM_{PS}$
	 & $aM^{\rm P-wave}_{N+K}$
	 & $aM^{\rm S-wave}_{N^*+K}$
	 & $aM^{\rm P-wave}_{N+K^*}$		\cr \hline
1.2780 & 1.949(31)  & 1.872(36)  & 1.692(7)  & 1.891(27)  & 1.873(9) \cr
1.2830 & 1.882(36)  & 1.816(40)  & 1.629(8)  & 1.830(32)  & 1.818(9) \cr
1.2885 & 1.802(44)  & 1.756(45)  & 1.558(8)  & 1.760(39)  & 1.755(10) \cr
1.2940 & 1.712(59)  & 1.693(56)  & 1.483(98) & 1.684(53)  & 1.690(11) \cr
1.2990 & 1.612(89)  & 1.624(80)  & 1.414(13) & 1.594(85)  & 1.631(14) \cr
1.3025 & 1.508(136) & 1.568(128) & 1.363(17) & 1.433(134) & 1.588(17) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I1.neg/MassS/tab.tex <==
\begin{table}[h]
\caption{\label{tab:difI1.neg}
	Mass differences between the $I(J^P)=1(\frac{1}{2}^-)$
	pentaquark and two-particle scattering states.}
\begin{ruledtabular} 
\begin{tabular}{c|ccc}
$\kappa$ & $aM_{NK(1)} - aM_{N+K}^{\rm S-wave}$
	 & $aM_{NK(2)} - aM_{N+K^*}^{\rm S-wave}$
	 & $aM_{SS} - aM_{N+K}^{\rm S-wave}$		\cr\hline
1.2780 & 0.080(13) &  0.058(10)  & --0.067(12) \cr
1.2830 & 0.089(14) &  0.052(11)  & --0.067(16) \cr
1.2885 & 0.095(15) &  0.042(13)  & --0.063(21) \cr
1.2940 & 0.097(23) &  0.029(19)  & --0.061(29) \cr
1.2990 & 0.100(45) &  0.009(27)  & --0.048(41) \cr
1.3025 & 0.143(52) & --0.006(46) & --0.114(74) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I1.neg/tab.tex <==
\begin{table}[h]     
\caption{\label{tab:I1.neg}
	Masses of the $I(J^P)=1(\frac{1}{2}^-)$ $NK$ and $SS$-type
	pentaquark states for various values of $\kappa$, compared
	with the masses of S-wave $N+K$ and $N+K^*$ two-particle states.}
\begin{ruledtabular} 
\begin{tabular}{c|ccccc}
$\kappa$ & $aM_{NK(1)}$ & $aM_{NK(2)}$ & $aM_{SS}$
	 & $aM_{N+K}$ & $aM_{N+K^*}$			\cr\hline
1.2780 & 1.635(11)  & 1.860(22)  & 1.678(12) & 1.556(9)  & 1.762(14) \cr
1.2830 & 1.558(14)  & 1.797(25)  & 1.601(14) & 1.487(10) & 1.704(16) \cr
1.2885 & 1.466(23)  & 1.721(31)  & 1.507(21) & 1.406(12) & 1.635(19) \cr
1.2940 & 1.374(39)  & 1.629(47)  & 1.401(35) & 1.317(17) & 1.561(26) \cr
1.2990 & 1.305(77)  & 1.577(77)  & 1.274(70) & 1.219(30) & 1.485(42) \cr
1.3025 & 1.237(140) & 1.554(175) & 1.197(98) & 1.140(46) & 1.421(68) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I1.pos/MassS/tab.tex <==
\begin{table}[h]     
\caption{\label{tab:difI1.pos}
	Mass differences between the $I(J^P)=1(\frac{1}{2}^+)$
        pentaquark and two-particle scattering states.}
\begin{ruledtabular} 
\begin{tabular}{c|cc}
$\kappa$ & $aM_{NK} - aM^{\rm P-wave}_{N+K}$
	 & $aM_{SS} - aM^{\rm P-wave}_{N+K}$ \cr\hline
1.2780 & 0.093(43) & 0.079(77) \cr
1.2830 & 0.079(53) & 0.046(95) \cr
1.2885 & 0.034(71) & 0.004(115) \cr
\end{tabular}
\end{ruledtabular}
\end{table}


==> TF_I1.pos/tab.tex <==
\begin{table}[h]
\caption{\label{tab:I1.pos}
	Masses of the $I(J^P)=1(\frac{1}{2}^+)$ colour-singlet $NK$
	and $SS$-type pentaquark states for various values of $\kappa$,
	compared with the masses of P-wave $N+K$, S-wave $N^* + K$
	and P-wave $N+K^*$ two-particle states.}
%	...[CHECK IF THIS TABLE IS CORRECT]...}
\begin{ruledtabular} 
\begin{tabular}{c|ccccc}
$\kappa$ & $aM_{NK}$ & $aM_{SS}$
	 & $aM^{\rm P-wave}_{N+K}$
	 & $aM^{\rm S-wave}_{N^*+K}$
	 & $aM^{\rm P-wave}_{N+K^*}$		\cr\hline
1.2780 & 1.864(30) & 1.764(80)  & 1.692(7)  & 1.891(27)  & 1.873(9) \cr
1.2830 & 1.800(37) & 1.667(99)  & 1.629(8)  & 1.830(32)  & 1.818(9) \cr
1.2885 & 1.731(45) & 1.553(118) & 1.558(8)  & 1.760(39)  & 1.755(10) \cr
1.2940 & 1.676(45) & 1.413(158) & 1.483(10) & 1.684(53)  & 1.690(11) \cr
1.2990 & 1.623(57) & 1.290(248) & 1.414(13) & 1.594(85)  & 1.631(14) \cr
1.3025 & 1.557(74) & 1.354(416) & 1.363(17) & 1.433(134) & 1.588(17) \cr
\end{tabular}
\end{ruledtabular}
\end{table}

